Bridging Gaps with Tensor Networks: From the Haldane Gap and Beyond

Proofs generated by large language models are often difficult to understand, generalize, or formalize directly. Here we verify, digest, and formalize OpenAI's computer-assisted proof of a uniform gap in the periodic spin-1 Heisenberg chain using tensor-network diagrams and Lean 4. Reading the partition-function network along space and imaginary time shows how finite-ring bounds propagate across doubled lengths and inverse temperatures to all longer even rings, sharpening the spin-1 bound from the same finite inputs by a factor of 19 to $\Delta_L > 0.0729$ for all even $L \geq 36$. We identify reflection positivity as the general condition behind the proof and certify uniform gaps in seven additional spin chains and ladders. More broadly, digesting machine-generated proofs into transparent physical mechanisms yields sharper bounds, broader theorems, and reusable formal verifications.

==> figures/diagrams-models.tex <==
% Diagrams for Supplemental Material Section SIV (reflection-positive models and seed certificates).
% Every macro carries one step of the structural classification or seed-certification argument.

% A staggered longitudinal field along a chain, matching \fieldsame and \fieldopp.
\newcommand{\fieldstag}{\tikz[baseline=0pt,x=1em,y=1em,line width=.45pt]{
 \draw[arxiv boundary] (0,.4)--(1.8,.4);
 \foreach \x/\s in {0/1,.6/-1,1.2/1,1.8/-1}{
   \fill (\x,.4) circle[radius=.08];
   \draw[arxiv small arrow,black!55,line width=.7pt]
     (\x,{.4-.36*\s})--(\x,{.4+.36*\s});}}}

% A pi rotation about y on every odd site (ticked) turns the staggered field
% into the uniform on-site term o = -h_st P_z, and each bond between a rotated
% and an unrotated site is one matched real pair across its mirror. Display
% figure; the pair itself is drawn beside it with \rpbondpic{P_\alpha}{P_\alpha}.
\newcommand{\staggerrotation}{\begin{tikzpicture}[x=1em,y=1em,font=\footnotesize,
  baseline={([yshift=-.5ex]current bounding box.center)}]
 \draw[arxiv boundary] (-.4,0)--(5.9,0);
 \foreach \x/\s/\t in {0/-1/1,1.1/1/0,2.2/-1/1,3.3/1/0,4.4/-1/1,5.5/1/0}{
  \fill (\x,0) circle[radius=.09];
  \draw[arxiv small arrow] (\x,{-.5*\s})--(\x,{.5*\s});
  \ifnum\t=1 \draw[arxiv boundary] (\x,-.75)--(\x,-1);\fi}
 \node[arxiv note,anchor=north] at (2.75,-1.1) {$-h_{\mathrm{st}}\sum_j(-1)^jS_j^z$};
 \draw[arxiv gray flow] (6.9,0)--(11.6,0) node[midway,above,arxiv note] {$u_y$ on odd sites};
 \draw[arxiv boundary] (12.2,0)--(18.5,0);
 \foreach \x in {12.6,13.7,14.8,15.9,17,18.1}{
  \fill (\x,0) circle[radius=.09];
  \draw[arxiv small arrow] (\x,-.5)--(\x,.5);}
 \draw[arxiv bond] (14.8,0)--(15.9,0);
 \draw[arxiv mirror] (15.35,-.75)--(15.35,.75);
 \node[arxiv note,text=mpoblue,anchor=north] at (15.35,-1.1) {$o=-h_{\mathrm{st}}P_z$};
\end{tikzpicture}}


% Two-site unit cell (a,b) with internal swap F across an inter-cell mirror cut:
% C_\alpha acts on the right spin b of the left cell, and F C_\alpha F acts on its
% mirror image, the left spin a of the right cell.
% Site labels sit below the legs, outside the cells, so nothing crosses a box.
\newcommand{\cellbondform}{\tikz[tn,tn centered]{
 \draw[arxiv cell] (-3.3,-.95) rectangle (1.1,.95);
 \draw[arxiv cell] (2.4,-.95) rectangle (7.1,.95);
 \foreach \x/\l in {-2.2/a,0/b,3.8/a,6/b}{
  \draw[phys] (\x,-1.3)--(\x,1.3);
  \node[font=\scriptsize,arxiv note,anchor=north,inner sep=1pt] at (\x,-1.35) {$\l$};}
 \draw[mpored] (0,0)--(3.8,0);
 \draw[arxiv mirror] (1.75,-1.45)--(1.75,1.45);
 \node[xop,fill=white] at (0,0) {$C_\alpha$};
 \node[xop,fill=white] at (3.8,0) {$FC_\alpha F$};}}

% Internal mirror cut across the intra-cell bond of a reflection-positive dimer
% cell (a,b), factoring the one-cell spatial transfer operator as K K^T >= 0.
\newcommand{\oddcellpos}{\tikz[tn,tn centered]{
 \draw[arxiv cell] (-2.7,-.95) rectangle (2.7,.95);
 \draw[phys] (-1.3,-1.3)--(-1.3,1.3) (1.3,-1.3)--(1.3,1.3);
 \draw[mpored] (-3.6,0)--(3.6,0);
 \draw[arxiv mirror] (0,-1.45)--(0,1.45);
 \node[xop,fill=white] at (-1.3,0) {$K$};
 \node[xop,fill=white] at (1.3,0) {$K^{\mathsf T}$};}}

% Rung cell of a two-leg ladder across an inter-cell mirror cut: the reflection
% keeps each leg on its own side (F = I), so C_{1,alpha} on leg 1 and C_{2,alpha}
% on leg 2 each face their own copy, and the rung interaction, even under the
% reflection, sits in the on-site box o. Twin of \cellbondform; a bond line hops
% over the other leg's wire where it has no vertex.
\newcommand{\rungcellform}{\tikz[tn,tn centered]{
 \draw[arxiv cell] (-3.7,-1.95) rectangle (1.4,1.95);
 \draw[arxiv cell] (2.4,-1.95) rectangle (7.5,1.95);
 \foreach \x/\l in {-2.3/1,0/2,3.8/1,6.1/2}{
  \draw[phys] (\x,-2.3)--(\x,2.3);
  \node[font=\scriptsize,arxiv note,anchor=north,inner sep=1pt] at (\x,-2.35) {$\l$};}
 \node[gibbs,minimum width=3.6em] at (-1.15,0) {$o$};
 \node[gibbs,minimum width=3.6em] at (4.95,0) {$o$};
 \draw[arxiv bond] (-2.3,1.25)--(-.3,1.25)
  arc[start angle=180,end angle=0,radius=.3]--(3.8,1.25);
 \draw[arxiv bond] (0,-1.25)--(3.5,-1.25)
  arc[start angle=180,end angle=0,radius=.3]--(6.1,-1.25);
 \draw[arxiv mirror] (1.9,-2.45)--(1.9,2.45);
 \node[xop,fill=white] at (-2.3,1.25) {$C_{1,\alpha}$};
 \node[xop,fill=white] at (3.8,1.25) {$C_{1,\alpha}$};
 \node[xop,fill=white] at (0,-1.25) {$C_{2,\alpha}$};
 \node[xop,fill=white] at (6.1,-1.25) {$C_{2,\alpha}$};
 \node[font=\scriptsize,arxiv note,anchor=south,inner sep=1pt] at (1.9,2.5) {$F=\smI$};}}

% Spin-1 bilinear-biquadratic phase circle showing the reflection-positive arc
% [-pi + arctan 2, 0] (teal, admissible), the Haldane sub-arc (-pi/4, 0] where the
% bootstrap applies (dashed gray), and the special points.
\newcommand{\blbqcircle}{\begin{tikzpicture}[x=1.05cm,y=1.05cm,font=\footnotesize]
 \def\R{1.2}
 \draw[arxiv axis line] (0,0) circle[radius=\R];
 \draw[tncert,line width=2.2pt] (0:\R) arc[start angle=0,end angle=-116.57,radius=\R];
 \draw[black!55,densely dashed,line width=2.2pt] (0:{\R+.12}) arc[start angle=0,end angle=-45,radius={\R+.12}];
 \foreach \a in {45,90,-45,-135}{\draw[black!55,line width=.45pt] (\a:{\R-.12})--(\a:{\R+.12});}
 \node[arxiv strong note] at (-22:{\R+.75}) {Haldane};
 \node[arxiv strong note] at (67.5:{\R+.38}) {critical};
 \node[arxiv strong note] at (180:{\R+.42}) {FM};
 \node[arxiv strong note] at (-90:{\R+.38}) {dimerized};
 \foreach \a in {0,18.43,45,-45,-116.57}{\fill (\a:\R) circle[radius=1.3pt];}
 \node[anchor=west] at (18.43:{\R+.08}) {AKLT};
 \node[anchor=west] at ([yshift=-1pt]0:{\R+.2}) {Heisenberg ($\vartheta=0$)};
 \node[anchor=south west] at (45:{\R+.02}) {ULS};
 \node[anchor=north west] at (-45:{\R+.26}) {TB};
 \node[anchor=north east] at (-116.57:{\R+.02}) {$-\pi{+}\arctan2$};
 \draw[arxiv gray flow] (0,0)--(35:.58) node[pos=1.18,arxiv note] {$\vartheta$};
\end{tikzpicture}}

% Half-length seed lift (spin1_largeD, stage 2): the spectra at lengths n_0
% and 2n_0 give three purities. Squaring in space at beta_0 and at 2beta_0
% bounds both spatial purities at 2n_0; the torus identity at length 2n_0,
% with P_s(2n_0,beta_0) <= 1 dropped, bounds the thermal purity at 4n_0. The
% pair (f(s), 1-(1-f(s_2))(1-t)^2) is the seed at 2n_0; no ring of length
% 4n_0 is diagonalized.
\newcommand{\halflengthlift}{\begin{prooflanes}[5.2]\def\lanedy{1.1}
 \lanebound{s}{hs0}{0}{0}{$\Ps(n_0,\beta_0)\ge1-s,\quad\Ps(n_0,2\beta_0)\ge1-s_2$}
 \lanebound{t}{ht0}{1}{0}{$\Pt(2n_0,\beta_0)\ge1-t$}
 \lanebound{s}{hs1}{0}{1}{$\Ps(2n_0,\beta_0)\ge1-f(s),\quad\Ps(2n_0,2\beta_0)\ge1-f(s_2)$}
 \lanebound{t}{ht1}{1}{1.6}{$\Pt(4n_0,\beta_0)\ge(1-f(s_2))(1-t)^2$}
 \lanemove[mpored]{hs0}{hs1}{1}{square in space at $\beta_0$ and $2\beta_0$}
 \lanemove{ht0}{ht1}{2}{identity~\eqref{models:eq:half-length} at $2n_0$}
 \laneuse{hs1}{2}
 \lanetag[above]{hs0}{spectra at $n_0$ and $2n_0$, at $\beta_0$ and $2\beta_0$}
 \lanetag[above]{ht0}{spectrum at $2n_0$}
 \lanetag[below]{hs1}{seed at $2n_0$: $p_0=f(s)$}
 \lanetag[below]{ht1}{seed at $2n_0$: $q_0=1-(1-f(s_2))(1-t)^2$}
\end{prooflanes}}

% Spectral sandwich used in the unconditional Lean-kernel proof for the
% mixed-field Ising chain at L in {6,12}: two residual intervals near E_0, E_1
% and a configuration-counting threshold rho bounding all remaining 2^L - 2 levels.
% Read along the eigenvalue axis: two certified intervals, the empty band up to
% the counting threshold rho, and the bulk of levels at or above rho.
\newcommand{\isingsandwich}{\begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize]
 \draw[arxiv axis line,-{Latex[length=1.4mm]}] (0,0)--(11.6,0)
  node[anchor=west,arxiv note] {$\lambda$};
 \foreach \x/\i in {1.1/0,3.4/1}{
  \draw[tncert,line width=.45pt] (\x-.35,-.18) rectangle (\x+.35,.18);
  \fill[tncert] (\x,0) circle[radius=1.3pt];
  \node[anchor=south,arxiv cert note] at (\x,.26) {$\lambda_\i\in[\theta_\i\pm\delta]$};
  \node[anchor=north,arxiv note] at (\x,-.26) {trial $x_\i$};}
 \fill[arxiv exclude band] (4.1,-.12) rectangle (7.1,.12);
 \node[anchor=south,arxiv exclude note] at (5.6,.2) {no eigenvalue};
 \node[anchor=north,arxiv exclude note] at (5.4,-.2) {$|B|=2$ below $\rho$};
 \draw[black!70,line width=.7pt] (7.1,-.28)--(7.1,.28);
 \node[anchor=north,arxiv strong note] at (7.1,-.3) {$\rho$};
 \foreach \x in {7.5,7.85,8.15,8.5,8.9,9.35,9.85,10.3,10.75}{
  \draw[arxiv axis line] (\x,-.12)--(\x,.12);}
 \node[anchor=south,arxiv note] at (9.1,.2) {$2^L-2$ eigenvalues $\lambda_i\ge\rho$};
 \node[anchor=north,arxiv note] at (9.1,-.26) {diagonal count~\eqref{models:eq:gershgorin}};
\end{tikzpicture}}

% A classical Ising configuration on a ring segment, one arrow per spin; a
% dashed tick marks each domain wall between opposite neighbors. Carries the
% counting fact: only the two uniform configurations have no wall.
\newcommand{\spinrow}[1]{\tikz[baseline=0pt,x=1em,y=1em]{
 \xdef\tnprev{0}
 \foreach \s [count=\i from 0] in {#1}{
  \draw[arxiv small arrow] ({.42*\i},{.42-.32*\s})--({.42*\i},{.42+.32*\s});
  \ifnum\i>0 \ifnum\tnprev=\s\else
   \draw[arxiv identified] ({.42*\i-.21},-.02)--({.42*\i-.21},.86);\fi\fi
  \xdef\tnprev{\s}}}}

% The eight certified seeds of Table S2 in the (p_0, q_0) plane against the
% admissible region of the asymmetric recurrence (boundary: the update of
% Eq. sm:eq:update iterated in floating point until both defects fall below
% 1/100; p_0 may reach 0.217 at q_0 -> 0 and q_0 may reach 0.200 at p_0 -> 0)
% and the symmetric threshold eps_* = 0.1273 (dashed). Seeds are numbered in
% the key; the D = 4 point is plotted at the values printed in the table.
\newcommand{\seedscatter}{\begin{tikzpicture}
 \begin{axis}[arxiv axis,xmode=log,ymode=log,width=10.5cm,height=6cm,
  xmin=2e-6,xmax=1,ymin=6e-6,ymax=1,clip=false,
  xlabel={\textcolor{mpored}{$p_0\ge1-\Ps(n_0,\beta_0)$ (spatial)}},
  ylabel={\textcolor{mpoblue}{$q_0\ge1-\Pt(2n_0,\beta_0)$ (thermal)}},
  xlabel near ticks,ylabel near ticks]
  \addplot[arxiv curve,draw=tncert] coordinates {
   (2e-6,6e-6) (2e-6,0.2006) (0.0001,0.2006) (0.001,0.2003) (0.003,0.1997)
   (0.006,0.1988) (0.01,0.1975) (0.015,0.1958) (0.02,0.194) (0.03,0.1902)
   (0.04,0.186) (0.05,0.1813) (0.06,0.1762) (0.07,0.1706) (0.08,0.1645)
   (0.09,0.1579) (0.1,0.1506) (0.11,0.1427) (0.12,0.1341) (0.13,0.1247)
   (0.14,0.1145) (0.15,0.1035) (0.16,0.09152) (0.17,0.07852) (0.18,0.06442)
   (0.19,0.04913) (0.2,0.03255) (0.205,0.02375) (0.21,0.01459)
   (0.215,0.005041) (0.217,0.001114) (0.2175,6e-6)};
  \draw[arxiv guide] (axis cs:2e-6,0.12731)--(axis cs:0.12731,0.12731)
   --(axis cs:0.12731,6e-6);
  \node[arxiv note,anchor=south west] at (axis cs:2.6e-6,0.135) {$\varepsilon_*$};
  \node[arxiv cert note,anchor=west] at (axis cs:2.6e-6,1.5e-4) {admissible: recurrence converges};
  \node[arxiv exclude note,anchor=south] at (axis cs:3e-3,0.4) {diverges};
  \addplot[only marks,mark=*,mark size=1.3pt,tncert] coordinates {
   (6.937e-4,7.327e-4) (1.133e-2,1.224e-2) (4.972e-2,3.206e-2)
   (3.633e-3,3.141e-2) (3.509e-2,2.463e-2) (1.125e-1,5.162e-2)
   (9.064e-6,3.141e-5) (3.054e-2,4.796e-2)};
  % direct labels; the crowded top-right cluster gets short leaders to the right margin
  \node[arxiv strong note,anchor=west,inner sep=2.5pt] at (axis cs:6.937e-4,7.327e-4) {staggered field};
  \node[arxiv strong note,anchor=east,inner sep=2.5pt] at (axis cs:1.133e-2,1.224e-2) {dimerized $S=\tfrac12$};
  \node[arxiv strong note,anchor=east,inner sep=2.5pt] at (axis cs:3.633e-3,3.141e-2) {single-ion $D=4$};
  \node[arxiv strong note,anchor=west,inner sep=2.5pt] at (axis cs:9.064e-6,3.141e-5) {mixed-field Ising};
  \draw[arxiv boundary,line width=.3pt] (axis cs:4.972e-2,3.206e-2)--(axis cs:1.6,1.3e-2);
  \node[arxiv strong note,anchor=west,inner sep=2pt] at (axis cs:1.6,1.3e-2) {dimerized $S=1$};
  \draw[arxiv boundary,line width=.3pt] (axis cs:3.509e-2,2.463e-2)--(axis cs:1.6,5e-3);
  \node[arxiv strong note,anchor=west,inner sep=2pt] at (axis cs:1.6,5e-3) {Heisenberg ladder};
  \draw[arxiv boundary,line width=.3pt] (axis cs:1.125e-1,5.162e-2)--(axis cs:1.6,9e-2);
  \node[arxiv strong note,anchor=west,inner sep=2pt] at (axis cs:1.6,9e-2) {Ising ladder};
  \draw[arxiv boundary,line width=.3pt] (axis cs:3.054e-2,4.796e-2)--(axis cs:1.6,3.3e-1);
  \node[arxiv strong note,anchor=west,inner sep=2pt] at (axis cs:1.6,3.3e-1) {Heisenberg $S=1$};
 \end{axis}
\end{tikzpicture}}


==> figures/diagrams-obc.tex <==
% Diagrams for the open-chain section of the Supplemental Material.
% All coordinates in tn pictures are in em; standalone pictures use cm.

% Folded contraction: the upper row is a ket, the lower row its adjoint,
% so the contraction is a squared norm (from thermal-mpo-gap-note.tex).
\newcommand{\folded}[1]{\tikz[tn,tn centered]{
 \begin{scope}[yshift=.8em]\tnchainpath[capr=v_j,name=u]{#1}\end{scope}
 \begin{scope}[yshift=-.8em]\tnchainpath[capr=\bar v_j,name=d]{#1}\end{scope}
 \draw[rounded corners=3pt] (u-L)--++(-.35em,0)|-(d-L);}}

% A middle operator of norm at most one lets Cauchy-Schwarz bound an open
% signed contraction by the squared norm of its caps, which is the folded
% even-length pair: |<ybar| R^{n-M} U_P |y>| <= ||y||^2. Use in math mode.
\newcommand{\schwarzfold}{\left|\,\tikz[tn,tn centered]{
  \tnchainpath[node=sym,capl={\bar y},capr={y},name=m]{R_j^{n-M}U_P}
  \node[arxiv note,font=\scriptsize,anchor=south,inner sep=1.5pt] at (m-1.north)
   {$\|\cdot\|\le1$};}\,\right|
 \le\folded{R_j^{M/2}}}

% \cancelled[color]{glyph}: a term struck through because it cancels.
\newcommand{\cancelled}[2][black!60]{\tikz[baseline=(n.base)]{
 \node[inner sep=1pt] (n) {#2};
 \draw[#1,line width=.7pt] ([xshift=1pt]n.south west)--([xshift=-1pt]n.north east);}}

% The three tracked contractions: ring purity, boundary overlap, thermal purity.
\newcommand{\obcring}{\tnchain[node=xvertex,ring]{,\cdots,}}
\newcommand{\obcends}{\tnchain[capl={\bar v},capr={v}]{\Pi}}
\newcommand{\obcthermal}{\tncolumn[ring]{\rho^{\opp},\rho^{\opp}}}

% Boundary caps as z-events on the end worldlines (grey: boundary objects):
% each event is a rung from the cap to the end site at its time. The conjugated left cap weights each
% event by -ih and the plain right cap by +ih, so the two endpoint fields are
% opposite; with #1=1 the rotation U_P on the right cap negates its events
% and the fields become equal.
\newcommand{\capfields}[1]{\tikz[tn,tn centered,font=\scriptsize]{
 \draw[phys] (0,-1.8)--(0,1.8);
 \draw[phys] (6.4,-1.8)--(6.4,1.8);
 \node[anchor=south,inner sep=2pt] at (0,1.8) {site $1$};
 \node[anchor=south,inner sep=2pt] at (6.4,1.8) {site $n$};
 \draw[mpored] (0,-.1)--(1.6,-.1); \draw[mpored] (4.8,.3)--(6.4,.3);
 \node[xvertex] at (0,-.1) {}; \node[xvertex] at (6.4,.3) {};
 \foreach \d in {-.3,0,.3}{\fill (3.2+\d,.1) circle[radius=.06];}
 % left cap: conjugated, events weighted by -ih
 \node[bvec,label=left:{$\bar v_\beta$}] (l) at (-3,0) {};
 \draw[arxiv boundary] (l)--(0,1); \draw[arxiv boundary] (l)--(0,-1);
 \fill[arxiv leading weight] (0,1) circle[radius=.12]; \fill[arxiv leading weight] (0,-1) circle[radius=.12];
 \node[anchor=south east,inner sep=1pt,arxiv note] at (-.2,1.08) {$-ih\,G_z$};
 \node[anchor=north east,inner sep=1pt,arxiv note] at (-.2,-1.08) {$-ih\,G_z$};
 % right cap: plain (or rotated by U_P), events weighted by +ih (or -ih)
 \ifnum#1=1
  \node[sym,label=right:{$U_Pv_\beta$}] (r) at (9.4,0) {$U_P$};
  \def\rsign{-}
 \else
  \node[bvec,label=right:{$v_\beta$}] (r) at (9.4,0) {};
  \def\rsign{+}
 \fi
 \draw[arxiv boundary] (6.4,1)--(r); \draw[arxiv boundary] (6.4,-1)--(r);
 \fill[arxiv leading weight] (6.4,1) circle[radius=.12]; \fill[arxiv leading weight] (6.4,-1) circle[radius=.12];
 \node[anchor=south west,inner sep=1pt,arxiv note] at (6.6,1.08) {$\rsign ih\,G_z$};
 \node[anchor=north west,inner sep=1pt,arxiv note] at (6.6,-1.08) {$\rsign ih\,G_z$};
 % the field each end contributes to the Hamiltonian
 \node[anchor=north,inner sep=2pt] at (0,-1.8) {$-hS_1^z$};
 \node[anchor=north,inner sep=2pt] at (6.4,-1.8) {$\rsign hS_n^z$};}}

% The local tensor is one site worldline with an event at every bond rung,
% and the time ordering runs over both bonds together: the product follows
% the interleaved times, not the side, so the traced kernel is symmetric,
% X_beta(a,b) = X_beta(b,a). Display figure (open chains, local tensor).
\newcommand{\worldlinekernel}{\begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize]
 % imaginary time runs upward along the worldline
 \draw[arxiv thermal flow] (-.6,.1)--(-.6,1.9) node[above,inner sep=1pt] {$\tau$};
 % the open worldline of W (left) and its physical trace X (right)
 \foreach \x/\closed in {1.3/0,5.5/1}{
  \draw[phys] (\x,0)--(\x,2);
  \ifnum\closed=1
   \draw[phys,ring] (\x,2)--(\x,2.3)--(\x+.8,2.3)--(\x+.8,-.3)--(\x,-.3)--(\x,0);
  \else
   \node[anchor=south,inner sep=2pt] at (\x,2) {$\langle s|$};
   \node[anchor=north,inner sep=2pt] at (\x,0) {$|s'\rangle$};
  \fi
  % rungs: a enters from the left at tau_1 and tau_3, b from the right at tau_2
  \foreach \y/\s/\g/\a in {.5/-1/G_x/south west,1/1/G_z/south east,1.5/-1/G_y/south west}{
   \draw[arxiv bond] (\x,\y)--({\x+\s*1.2},\y);
   \node[xvertex] at (\x,\y) {};
   \node[anchor=\a,inner sep=1.5pt] at ({\x-\s*.07},\y) {$\g$};}}
 \node[arxiv note,anchor=east,inner sep=2pt] at (.1,.5) {$\tau_1$};
 \node[arxiv note,anchor=west,inner sep=2pt] at (2.5,1) {$\tau_2$};
 \node[arxiv note,anchor=east,inner sep=2pt] at (.1,1.5) {$\tau_3$};
 \node[text=mpored,anchor=south,inner sep=1.5pt] at (.6,1.5) {$a$};
 \node[text=mpored,anchor=south,inner sep=1.5pt] at (2.1,1) {$b$};
 \node[text=mpored,anchor=south,inner sep=1.5pt] at (4.8,1.5) {$a$};
 \node[text=mpored,anchor=south,inner sep=1.5pt] at (6.55,1) {$b$};
 \node[anchor=north,inner sep=2pt] at (1.3,-.5)
  {$W_\beta^{ss'}(a,b)=\langle s|G_yG_zG_x|s'\rangle$};
 \node[anchor=north,inner sep=2pt] at (5.7,-.5)
  {$X_\beta(a,b)=\Tr(G_yG_zG_x)$};
 \draw[arxiv gray flow] (3.1,1)--(3.9,1) node[midway,above,arxiv note] {$\sum_s$};
\end{tikzpicture}}

% One induction step in the (length, inverse temperature) plane: Step 1
% (grey, boundary) compares two lengths at the new temperature, Step 2 (red,
% space) doubles the length at the old temperature using the Step 1 output,
% Step 3 (blue, time) squares in imaginary time.
\newcommand{\obcstairs}{\begin{tikzpicture}[x=1cm,y=1cm,
 every node/.style={arxiv label,inner sep=1pt},
 ept/.style={circle,draw=black!55,fill=white,inner sep=2pt},
 tpt/.style={circle,draw=mpoblue,fill=white,inner sep=2pt}]
 % no grid: the points and the tick labels locate the three moves
 \foreach \x/\l in {0/{M_j/2},1.4/{M_j},4.2/{2M_j}}{\node[anchor=north] at (\x,-.22) {$\l$};}
 \node[anchor=east] at (-.35,.2) {$\beta_j$};
 \node[anchor=east] at (-.35,1.6) {$\beta_{j+1}$};
 % step 1: both lengths at the new temperature, overlap cancels
 \draw[black!55,densely dashed,line width=.7pt] (0,1.6)--(1.4,1.6);
 \draw[arxiv gray flow] (0,.12)--(0,1.48);
 \draw[arxiv gray flow] (1.4,.12)--(1.4,1.48);
 \node[lanemv] at (.7,1.05) {1};
 % step 2: double the length at the old temperature
 \draw[flow,mpored] (1.55,0)--(4.05,0);
 \node[lanemv] at (2.8,.42) {2};
 \draw[laneuse] (1.4,1.45)--(2.6,.55);
 % step 3: square in imaginary time
 \draw[flow,mpoblue] (4.2,.12)--(4.2,1.48);
 \node[lanemv] at (4.2,.8) {3};
 % points
 \node[ept] at (0,0) {}; \node[tpt] at (1.4,0) {};
 \node[ept] at (1.4,1.6) {}; \node[tpt] at (4.2,1.6) {};
 \node[ept,draw=black!25,fill=white] at (0,1.6) {};
 \node[anchor=south west,inner sep=2pt] at (.1,.1) {$e_{M_j/2}(j)$};
 \node[anchor=north,inner sep=2pt,text=mpoblue] at (2.8,-.06) {$\Pt^{\opp}(M_j,\beta_j)$};
 \node[anchor=south,inner sep=3pt] at (.7,1.66) {$e_{M_j}(j+1)$};
 \node[anchor=south,inner sep=3pt,text=mpoblue] at (4.2,1.66) {$\Pt^{\opp}(2M_j,\beta_{j+1})$};
 % what each move proves, keyed by its number: the step is these three bounds
 \begin{scope}[shift={(6.1,0)},every node/.style={arxiv label,inner sep=1pt,anchor=west}]
  \node[lanemv,anchor=center] at (0,1.6) {1};
  \node at (.3,1.6) {$e_{M_j}(j+1)\le\dfrac{q}{1-q}\Bigl[\dfrac{1}{(1-e_{M_j/2}(j))^2\,\Pt^{\opp}(M_j,\beta_j)}-1\Bigr]$,\quad $q\ge\|R_{j+1}\|^{M_j/2}$};
  \node[lanemv,anchor=center] at (0,.8) {2};
  \node at (.3,.8) {$\Pt^{\opp}(2M_j,\beta_j)\ge r_j^{M_j}\,[1-e_{M_j}(j+1)]\,\Pt^{\opp}(M_j,\beta_j)$};
  \node[lanemv,anchor=center] at (0,0) {3};
  \node at (.3,0) {$1-\Pt^{\opp}(2M_j,\beta_{j+1})\le f\bigl(1-\Pt^{\opp}(2M_j,\beta_j)\bigr)$};
 \end{scope}
\end{tikzpicture}}

% The length ladder of the open-chain scales: ring length n_j (red), open
% length M_j = 2 n_j (grey), and the defect length k_j (tick), to a common
% scale so that k_j = M_j/2 for j >= 3 and n_{j+1} = M_j are visible.
\newcommand{\obcscales}{\begin{tikzpicture}[x=.33cm,y=1.3cm,
 every node/.style={arxiv label,inner sep=1pt}]
 \foreach \j/\y/\b/\M/\k/\ks in {2/0/49/2/{1.1833}/142,3/-1/98/4/2/240,4/-2/196/8/4/480,5/-3/392/16/8/960}{
  \node[anchor=east] at (-1.2,\y) {$j=\j$};
  \node[anchor=east,arxiv note] at (-4.2,\y) {$\beta_j=\b$};
  \draw[black!25,line width=2.4pt] (0,\y)--(\M,\y);
  \pgfmathsetmacro\n{\M/2}
  \draw[mpored,line width=2.4pt] (0,\y)--(\n,\y);
  \draw[black!70,line width=.7pt] (\k,\y-.2)--(\k,\y+.2);
  \pgfmathtruncatemacro\Msites{\M*120}
  \pgfmathtruncatemacro\nsites{\M*60}
  \node[anchor=west,arxiv note] at (\M+.3,\y) {$M_j=\Msites$};
  \node[anchor=south] at (\k,\y+.2) {$k_j=\ks$};
  \node[anchor=north west,text=mpored] at (0,\y-.22) {$n_j=\nsites$};}
\end{tikzpicture}}

% The three open-chain defects over the initialization steps j=2..5 on a
% logarithmic scale: boundary defect E_j (grey), thermal defect eta_j (blue),
% ring defect eps_j (red), and the 0.01 threshold of the induction (teal).
\newcommand{\obcladder}{\begin{tikzpicture}[x=1.4cm,y=.78cm,font=\footnotesize]
 \def\Es{-.854,-.921,-1.796,-3}
 \def\etas{-.678,-.810,-1.585,-3}
 \def\epss{-1.284,-1.790,-2.801,-4.825}
 \draw[arxiv cert guide] (0,-2)--(3,-2)
  node[right,tncert] {$x_5=10^{-2}$};
 \foreach \v [count=\i from 0] in \Es{\ifnum\i>0 \draw[arxiv series,black!55] ({\i-1},\El)--(\i,\v);\fi
  \fill[arxiv leading weight] (\i,\v) circle[radius=1.3pt]; \xdef\El{\v}}
 \foreach \v [count=\i from 0] in \etas{\ifnum\i>0 \draw[arxiv series,mpoblue] ({\i-1},\etal)--(\i,\v);\fi
  \fill[mpoblue] (\i,\v) circle[radius=1.3pt]; \xdef\etal{\v}}
 \foreach \v [count=\i from 0] in \epss{\ifnum\i>0 \draw[arxiv series,mpored] ({\i-1},\epsl)--(\i,\v);\fi
  \fill[mpored] (\i,\v) circle[radius=1.3pt]; \xdef\epsl{\v}}
 \node[mpoblue,anchor=west] at (3.08,-2.7) {$\eta_j$ (thermal)};
 \node[arxiv boundary,anchor=west] at (3.08,-3.32) {$E_j$ (boundary)};
 \node[mpored,anchor=west] at (3.08,-4.825) {$\varepsilon_j$ (ring)};
 \foreach \j [count=\i from 0] in {2,3,4,5}{\node[arxiv note] at (\i,-5.3) {$\j$};}
 \foreach \m [count=\i from 0] in {240,480,960,1920}{\node[arxiv note] at (\i,-5.72) {$\m$};}
 \foreach \b [count=\i from 0] in {49,98,196,392}{\node[arxiv note] at (\i,-6.14) {$\b$};}
 \node[arxiv note,anchor=east] at (-.25,-5.3) {$j$};
 \node[arxiv note,anchor=east] at (-.25,-5.72) {$M_j$};
 \node[arxiv note,anchor=east] at (-.25,-6.14) {$\beta_j$};
\end{tikzpicture}}

% Odd lengths covered by the length intervals [M_j, 2M_j] (red: space),
% j >= 5, on a log_2 axis; the target odd length is teal (conclusion).
\newcommand{\oddcoverage}{\begin{tikzpicture}[x=1.5cm,y=1cm,font=\footnotesize]
 \draw[arxiv axis line] (-.3,0)--(3.6,0);
 \foreach \x/\l in {0/1920,1/3840,2/7680,3/15360}{
  \draw[arxiv axis line] (\x,-.08)--(\x,.08);
  \node[arxiv note,anchor=north] at (\x,-.1) {$\l$};}
 \foreach \x/\j/\y in {0/5/.6,1/6/.9,2/7/1.2}{
  \draw[mpored,line width=1pt] (\x+.03,\y)--(\x+.97,\y);
  \node[mpored,anchor=west] at (\x+1.03,\y) {$[M_\j,2M_\j]$ at $\beta_\j$};}
 \fill[tncert] (.0075,0) circle[radius=1.3pt];
 \node[tncert,anchor=south west] at (.03,.06) {$n=1921$, first odd length};
 \node[arxiv note,anchor=west] at (3.65,0) {$n$};
\end{tikzpicture}}

% One scale of the periodic argument at the open-chain scales, read left to
% right: the two identities (grey) and the two squarings (red: space, blue:
% time) carry the ring defect eps to 6 eps^2 at (n_{j+1}, beta_{j+1}).
\newcommand{\ringsteps}{\begin{tikzpicture}[x=1cm,y=1cm]
 % the thermal lane is staggered one column to the right, so that each
 % use arrow (the other lane's bound entering an identity) is a short diagonal
 \node[lane s] (s0) at (0,1.05) {$\Ps(n_j,\beta_j)\ge1-\varepsilon$};
 \node[lane so] (s1) at (4.5,1.05) {$\Ps(n_j,2\beta_j)\ge(1-\varepsilon)^3$};
 \node[lane s] (s2) at (9,1.05) {$\Ps(2n_j,2\beta_j)\ge1-6\varepsilon^2$};
 \node[lane t] (t0) at (4.5,0) {$\Pt(2n_j,\beta_j)\ge1-\varepsilon$};
 \node[lane to] (t1) at (9,0) {$\Pt(4n_j,\beta_j)\ge(1-\varepsilon)^2(1-6\varepsilon^2)$};
 \node[lane t] (t2) at (13.5,0) {$\Pt(4n_j,2\beta_j)\ge1-6\varepsilon^2$};
 \node[lanemv] (m1) at ($(s0.east)!.5!(s1.west)$) {1};
 \node[lanemv] (m2) at ($(s1.east)!.5!(s2.west)$) {2};
 \node[lanemv] (m3) at ($(t0.east)!.5!(t1.west)$) {3};
 \node[lanemv] (m4) at ($(t1.east)!.5!(t2.west)$) {4};
 \draw[black!55,line width=.45pt] (s0)--(m1); \draw[arxiv gray flow] (m1)--(s1);
 \draw[arxiv bond] (s1)--(m2); \draw[flow,mpored] (m2)--(s2);
 \draw[black!55,line width=.45pt] (t0)--(m3); \draw[arxiv gray flow] (m3)--(t1);
 \draw[mpoblue,line width=.45pt] (t1)--(m4); \draw[flow,mpoblue] (m4)--(t2);
 \draw[laneuse,shorten <=1pt,shorten >=.5pt] (t0.north west)--(m1);
 \draw[laneuse,shorten <=1pt,shorten >=.5pt] (s2.south west)--(m3);
 \node[maprule,anchor=south] at (m1.north) {identity};
 \node[maprule,anchor=south] at (m2.north) {square};
 \node[maprule,anchor=north] at (m3.south) {identity};
 \node[maprule,anchor=north] at (m4.south) {square};
\end{tikzpicture}}

% Two capped MPO rows at beta_j stacked in imaginary time (\obcstack) equal
% one capped row at beta_{j+1}=2 beta_j (\obcstackdouble): the boundary
% vectors are part of the operator, so squaring the open-chain Gibbs
% operator is exact, and the doubled row carries the vectors v_{beta_{j+1}}.
\newcommand{\obcstack}{\tikz[tn,tn centered]{
 \begin{scope}[yshift=.95em]
  \tnchainpath[node=mpo,legs=.95em,caps,name=u]{W_{\beta_j},\cdots,W_{\beta_j}}\end{scope}
 \begin{scope}[yshift=-.95em]
  \tnchainpath[node=mpo,legs=.95em,caps,name=d]{W_{\beta_j},\cdots,W_{\beta_j}}\end{scope}
 \node[anchor=south,inner sep=2pt] at ([yshift=.2em]u-L) {$\bar v_j$};
 \node[anchor=south,inner sep=2pt] at ([yshift=.2em]u-R) {$v_j$};
 \node[anchor=north,inner sep=2pt] at ([yshift=-.2em]d-L) {$\bar v_j$};
 \node[anchor=north,inner sep=2pt] at ([yshift=-.2em]d-R) {$v_j$};}}
\newcommand{\obcstackdouble}{\tnchain[node=mpo,legs=1.9em,
 item={minimum height=1.3em},capl={\bar v_{j+1}},capr={v_{j+1}}]
 {W_{\beta_{j+1}},\cdots,W_{\beta_{j+1}}}}

% A purity above 1-eps forces the largest weight p_0 (black!55) above the
% dashed half line; the tail z=1-p_0 (black!25) is below 1/2.
\newcommand{\dominantglyph}{\tikz[baseline=0pt,x=.34em,y=1.1em]{
 \fill[arxiv leading weight] (0,0) rectangle ++(.78,.9);
 \fill[arxiv remainder weight] (1,0) rectangle ++(.78,.07);
 \fill[arxiv remainder weight] (2,0) rectangle ++(.78,.04);
 \draw[arxiv baseline] (-.2,0)--(3,0);
 \draw[arxiv guide] (-.2,.5)--(3,.5);}}


==> figures/diagrams-seeds.tex <==
% Diagrams for the Supplemental Material section on finite seed certificates.
% Every macro carries one step of the seed argument; none is decorative.

% The traces of Table cert:tab:traces on a logarithmic scale, even n tall and
% odd n short: K_{b_0} has eigenvalues of both signs with nearly equal modulus.
\newcommand{\tracebars}{\tikz[baseline=0pt,x=.34em,y=1.1em]{
 \foreach \h [count=\i] in {1,.1,.78,.37,.68,.49,.63,.55,.6}{
  \fill[mpored!70] ({\i-1},0) rectangle ++(.78,\h);}
 \draw[arxiv baseline] (-.2,0)--(9,0);}}

% The half-Gibbs trace as a squared Frobenius norm: for the real symmetric
% A = exp(-b_0 H/2), Tr A^2 = sum_c ||A e_c||^2 (the lower box is the mirror image
% of the upper one), so every basis column is one Poisson recursion at b_0/2 and
% the rounding errors add column by column. Use in math mode.
\newcommand{\halfgibbstrace}{\tncolumn[ring]{A,A}
 =\sum_c\;\tikz[tn,tn centered]{
  \draw[phys] (0,-1.9)--(0,1.9);
  \draw[arxiv mirror] (-1.2,0)--(1.2,0);
  \node[gibbs] at (0,.78) {$A$};
  \node[gibbs] at (0,-.78) {$A$};
  \node[bvec,label=right:{$e_c$}] at (0,1.9) {};
  \node[bvec,label=right:{$e_c$}] at (0,-1.9) {};}}

% Signed spectrum of the spatial transfer operator at b_0: eigenvalues of both
% signs with nearly equal moduli, so the odd power sums nearly cancel and traces
% of both parities of n are needed. Word-sized, in the \specbars idiom.
\newcommand{\signedspectrum}{\tikz[baseline={([yshift=-.5ex]current bounding box.center)},
 x=.34em,y=.6em]{
 \foreach \h [count=\i] in {1,-.94,.45,-.4,.25,-.2,.12}{
  \fill[mpored!70] ({\i-1},0) rectangle ++(.78,\h);}
 \draw[arxiv baseline] (-.2,0)--(7,0);}}

% Six-site ring drawn at (#1,#2) inside a picture, twisted on its closing bond
% when #3=1 (the in-picture form of \seedring).
\newcommand{\seedringat}[3]{\begin{scope}[shift={(#1,#2)},x=.2cm,y=.2cm]
 \draw[black!70,line width=.45pt] (90:1)--(30:1)--(-30:1)
  --(-90:1)--(-150:1)--(150:1)--cycle;
 \ifnum#3=1
  \draw[mpored,line width=1.6pt] (150:1)--(90:1);
  \node[font=\scriptsize,text=mpored] at (-.95,1.1) {$\pi$};
 \fi
 \foreach \a in {90,30,-30,-90,-150,150}{
  \filldraw[draw=black!70,fill=white,line width=.45pt] (\a:1) circle (.12);}
\end{scope}}

% Character table of the four pi-rotation sectors against the plain and the
% P_z-twisted ring: the twist counts N_x and N_y with a minus sign, so the two
% traces are J_n+3N_n and J_n-N_n.
\newcommand{\sectortable}{\begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize]
 \foreach \x/\s in {0/J,1.3/N_x,2.6/N_y,3.9/N_z}{
  \node[draw=black!55,line width=.45pt,minimum width=.95cm,minimum height=.5cm,
   inner sep=2pt] at (\x,0) {$\s$};}
 \foreach \x in {0,1.3,2.6,3.9}{\node[arxiv strong note] at (\x,-.68) {$+$};}
 \foreach \x/\sgn in {0/+,1.3/-,2.6/-,3.9/+}{\node[arxiv strong note] at (\x,-1.38) {$\sgn$};}
 \seedringat{-1.35}{-.68}{0}
 \seedringat{-1.35}{-1.38}{1}
 \node[anchor=west] at (4.7,-.68) {$Z_n=J_n+3N_n$};
 \node[anchor=west] at (4.7,-1.38) {$Z_n(P)=J_n-N_n$};
 \node[anchor=north,arxiv note] at (2.6,-1.62) {identical spectra};
\end{tikzpicture}}

% Both filters against their certified totals (plotted in units of 10^3):
% nonnegativity makes each total a limit for every eigenvalue of its sector,
% and the shaded exterior rays beyond +-U (for J) and +-V (for N) are empty.
\newcommand{\filterpair}{\begin{tikzpicture}
 \begin{axis}[arxiv axis,name=fj,width=6.2cm,height=4.1cm,
  xmin=-1.12,xmax=1.12,ymin=0,ymax=620,
  xlabel={$\lambda$},ylabel={$F_J(\lambda)$},
  xtick={-1.00139,0,1.00139},xticklabels={$-U$,$0$,$U$},
  ytick={0,318.6},yticklabels={$0$,$B_J$},scaled y ticks=false,
  samples=300,domain=-1.12:1.12,clip mode=individual,clip=false]
  \fill[arxiv exclude band] (axis cs:1.00139,0) rectangle (axis cs:1.12,620);
  \fill[arxiv exclude band] (axis cs:-1.12,0) rectangle (axis cs:-1.00139,620);
  \addplot[arxiv cert guide] coordinates {(-1.12,318.6) (1.12,318.6)};
  \addplot[arxiv curve,restrict y to domain=0:640]
   {x^4*(7+17*x-280*x^2-185*x^3+1000*x^4)^2/1000};
  \node[arxiv cert note,anchor=south] at (axis cs:0,318.6)
   {total $B_J$};
  \node[arxiv exclude note,anchor=south] at (axis cs:-1.06,628) {no $\lambda$};
  \node[arxiv exclude note,anchor=south] at (axis cs:1.06,628) {no $\lambda$};
 \end{axis}
 \begin{axis}[arxiv axis,at={(fj.east)},anchor=west,xshift=1.9cm,width=6.2cm,height=4.1cm,
  xmin=-1,xmax=1,ymin=0,ymax=90,
  xlabel={$\lambda$},ylabel={$F_N(\lambda)$},
  xtick={-0.872,0,0.872},xticklabels={$-V$,$0$,$V$},
  ytick={0,48.17},yticklabels={$0$,$B_N$},scaled y ticks=false,
  samples=300,domain=-1:1,clip mode=individual,clip=false]
  \fill[arxiv exclude band] (axis cs:0.872,0) rectangle (axis cs:1,90);
  \fill[arxiv exclude band] (axis cs:-1,0) rectangle (axis cs:-0.872,90);
  \addplot[arxiv cert guide] coordinates {(-1,48.17) (1,48.17)};
  \addplot[arxiv curve,restrict y to domain=0:92] {x^4*(12-394*x^2+1000*x^4)^2/1000};
  \node[arxiv cert note,anchor=south] at (axis cs:0,48.17)
   {total $B_N$};
  \node[arxiv exclude note,anchor=south] at (axis cs:-0.936,91) {no $\lambda$};
  \node[arxiv exclude note,anchor=south] at (axis cs:0.936,91) {no $\lambda$};
 \end{axis}
\end{tikzpicture}}

% Convexity of t^r moves mass to the cap: shifting mass from a smaller entry to
% a larger one never lowers sum t_i^r, until q entries sit at the cap a (dashed)
% and the remainder m-qa sits in one entry.
\newcommand{\massmoves}{\tikz[baseline=0pt,x=.5em,y=1.1em,line width=.35pt]{
 \foreach \o/\ha/\hb/\hc/\ca in {0/.4/.35/.25/30,5.3/.6/.15/.25/55,10.6/.6/.4/0/55}{
  \fill[black!\ca] (\o,0) rectangle ++(.8,\ha);
  \fill[arxiv remainder weight] ({\o+1.15},0) rectangle ++(.8,\hb);
  \fill[arxiv remainder weight] ({\o+2.3},0) rectangle ++(.8,\hc);
  \draw[arxiv guide] ({\o-.2},.6)--({\o+3.5},.6);
  \draw[arxiv baseline] ({\o-.25},0)--({\o+3.55},0);}
 \foreach \o in {3.75,9.05}{\draw[arxiv small arrow] (\o,.3)--({\o+1.2},.3);}}}

% Capped-mass extremum at the sixth power, both sectors on one vertical scale:
% the J mass sits as one entry at the cap ell^12 plus a remainder, each N list
% as one entry at V^12 plus a remainder; the sixth power keeps only the capped
% entry; Eq. cert:eq:dominance-check adds the three surviving numbers.
\newcommand{\cappedmassfigure}{\begin{tikzpicture}[x=1cm,y=2.4cm,font=\footnotesize]
 \node[arxiv strong note,anchor=south] at (2.1,1.14) {$J$: mass $m_J\le1.0658$, bound $\ell^{12}$};
 \fill[arxiv leading weight] (0,0) rectangle (.5,.9881);
 \fill[arxiv remainder weight] (.8,0) rectangle (1.3,.0777);
 \draw[arxiv guide] (-.1,.9881)--(1.4,.9881);
 \node[anchor=south] at (.25,.9881) {$0.9881$};
 \node[anchor=south] at (1.05,.0777) {$0.0777$};
 \draw[arxiv baseline] (-.1,0)--(1.4,0);
 \draw[arxiv gray flow] (1.7,.45)--(2.6,.45) node[midway,above] {$u\mapsto u^6$};
 \fill[arxiv leading weight] (2.9,0) rectangle (3.4,.9305);
 \node[anchor=south] at (3.15,.9305) {$0.9305$};
 \draw[arxiv baseline] (2.8,0)--(4.3,0);
 \begin{scope}[xshift=5.6cm]
  \node[arxiv strong note,anchor=south] at (2.1,1.14) {each $N$ list: mass $m_N\le0.2784$, bound $V^{12}$};
  \fill[arxiv bulk weight] (0,0) rectangle (.5,.1933);
  \fill[arxiv bulk weight] (1.1,0) rectangle (1.6,.0851);
  \draw[arxiv guide] (.55,.1933)--(.8,.1933);
  \node[anchor=south] at (.25,.1933) {$0.1933$};
  \node[anchor=south] at (1.35,.0851) {$0.0851$};
  \draw[arxiv baseline] (-.1,0)--(1.7,0);
  \draw[arxiv gray flow] (1.7,.45)--(2.6,.45) node[midway,above] {$u\mapsto u^6$};
  \node[anchor=south] at (3.55,0) {$<5.3\times10^{-5}$};
  \draw[arxiv baseline] (2.8,0)--(4.3,0);
 \end{scope}
\end{tikzpicture}}

% The lift from b_0 to b=rb_0: the trace bound M_k, split into its J share
% (dark) and the three N lists (light), is raised to the power r by
% sum z^r <= (sum z)^r, so the lifted total is D=M_k^r and the lifted J share
% is at most tau=(D+3E)/4 with E=J_k^r bounding the twisted trace.
\newcommand{\liftbars}{\begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize]
 \fill[arxiv leading weight] (0,0) rectangle (.45,.7);
 \fill[arxiv remainder weight] (0,.7) rectangle (.45,1.25);
 \draw[arxiv baseline] (-.1,0)--(.55,0);
 \node[anchor=east] at (-.05,.35) {$J$ share $\mathcal J_k$};
 \node[anchor=east] at (-.05,.98) {$N$ lists $3\mathcal N_k$};
 \node[anchor=south] at (.22,1.3) {$Z_k(b_0)\le M_k$};
 \node[anchor=north,arxiv note] at (.22,-.05) {at $b_0$};
 \draw[arxiv thermal flow] (1.3,.65)--(3.1,.65)
  node[midway,above,text=black] {$\sum_i z_i^r\le\bigl(\sum_i z_i\bigr)^r$};
 \fill[arxiv leading weight] (3.5,0) rectangle (3.95,.9);
 \fill[arxiv remainder weight] (3.5,.9) rectangle (3.95,1.55);
 \draw[arxiv baseline] (3.4,0)--(4.05,0);
 \node[anchor=west] at (4.0,.45) {$J$ share $\le\tau$};
 \node[anchor=south] at (3.72,1.6) {$Z_k(b)\le D=M_k^r$};
 \node[anchor=north,arxiv note] at (3.72,-.05) {at $b=rb_0$};
\end{tikzpicture}}

% Weight forcing at the lifted temperature: were every k-th power weight below
% the threshold t (dashed), the 120-site power sum would be at most D t^{2h-1}<1,
% so one weight w_0 exceeds t; three copies of such a weight in N would already
% exceed the total D, so w_0 lies in J.
\newcommand{\weightforcing}{\begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize]
 \foreach \h [count=\i from 0] in {.5,.4,.3,.2,.15}{
  \fill[arxiv remainder weight] ({.35*\i},0) rectangle ++(.27,\h);}
 \draw[arxiv baseline] (-.1,0)--(1.85,0);
 \draw[arxiv cert guide] (-.1,.6)--(1.85,.6) node[right] {$t$};
 \node[anchor=north,arxiv note,align=center] at (.85,-.05)
  {all $w_i\le t$:\\$\sum_iw_i^{2h}\le Dt^{2h-1}<1$};
 \begin{scope}[xshift=3.9cm]
  \fill[arxiv leading weight] (0,0) rectangle (.27,1.15);
  \foreach \h [count=\i from 1] in {.3,.2,.15,.1}{
   \fill[arxiv remainder weight] ({.35*\i},0) rectangle ++(.27,\h);}
  \draw[arxiv baseline] (-.1,0)--(1.85,0);
  \draw[arxiv cert guide] (-.1,.6)--(1.85,.6) node[right] {$t$};
  \node[anchor=south] at (.135,1.17) {$w_0$};
  \node[anchor=north,arxiv note,align=center] at (.85,-.05)
   {so some $w_0>t$,\\since $\sum_iw_i^{2h}=Z_{120}(b)>1$};
 \end{scope}
 \begin{scope}[xshift=7.8cm]
  \foreach \i in {0,1,2}{
   \filldraw[arxiv bulk box] (0,{.45*\i}) rectangle (.27,{.45*\i+.45});
   \node[anchor=east] at (-.05,{.45*\i+.22}) {$t$};}
  \draw[arxiv baseline] (-.1,0)--(1.1,0);
  \draw[arxiv guide] (.35,1.05)--(1.1,1.05) node[right] {$D$};
  \node[anchor=north,arxiv note,align=center] at (.5,-.05)
   {three copies in $N$:\\$3t>D$, so $w_0\in J$};
 \end{scope}
\end{tikzpicture}}

% The residual moment after removing w_0 is convex in the J remainder x, so its
% maximum sits at an endpoint: x=0 (all residual mass D-t in the N lists) or
% x=tau-t (the J remainder full, D-tau left for the N lists).
\newcommand{\residualends}{\begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize]
 \draw[arxiv dotted guide] (0,0) rectangle (.27,.75);
 \foreach \i in {1,2,3}{
  \filldraw[arxiv bulk box] ({.35*\i},0) rectangle ++(.27,.6);}
 \draw[arxiv baseline] (-.1,0)--(1.45,0);
 \node[anchor=north,arxiv note] at (.135,-.05) {$x=0$};
 \node[anchor=west,arxiv note] at (1.45,.3) {$\tfrac{D-t}3$ each};
 \node[anchor=south] at (.7,.8) {$3\bigl(\tfrac{D-t}3\bigr)^s$};
 \node[arxiv note] at (3.3,.4) {or};
 \begin{scope}[xshift=4cm]
  \fill[arxiv leading weight] (0,0) rectangle (.27,.75);
  \foreach \i in {1,2,3}{
   \filldraw[arxiv bulk box] ({.35*\i},0) rectangle ++(.27,.35);}
  \draw[arxiv baseline] (-.1,0)--(1.45,0);
  \node[anchor=north,arxiv note] at (.135,-.05) {$x=\tau-t$};
  \node[anchor=west,arxiv note] at (1.45,.3) {$\tfrac{D-\tau}3$ each};
  \node[anchor=south] at (.7,.8) {$(\tau-t)^s+3\bigl(\tfrac{D-\tau}3\bigr)^s$};
 \end{scope}
\end{tikzpicture}}

% Refinement: once w_0 > t, Eq. cert:eq:refinement raises the threshold to t'.
\newcommand{\thresholdup}{\tikz[baseline=0pt,x=.5em,y=1.1em,line width=.35pt]{
 \fill[arxiv leading weight] (0,0) rectangle (.8,1);
 \foreach \h [count=\i from 1] in {.25,.15,.1}{
  \fill[arxiv remainder weight] ({1.15*\i},0) rectangle ++(.8,\h);}
 \draw[arxiv baseline] (-.25,0)--(4.9,0);
 \draw[arxiv cert guide] (-.25,.45)--(4.9,.45);
 \draw[arxiv cert guide] (-.25,.8)--(4.9,.8);
 \draw[arxiv small arrow,tncert] (4.5,.48)--(4.5,.77);}}

% Ordered Boltzmann weights of the 120-site ring at b_0: the ground weight z_0
% exceeds one (dotted line) and the others share at most M_120 - 1.
\newcommand{\boltzmannbars}{\tikz[baseline=0pt,x=.34em,y=1.1em]{
 \foreach \h [count=\i] in {1,.22,.12,.07}{
  \fill[mpoblue] ({\i-1},0) rectangle ++(.78,\h);}
 \draw[arxiv baseline] (-.2,0)--(4,0);
 \draw[arxiv dotted guide] (-.2,.7)--(4,.7);}}

% Finite-prefix coverage of even lengths for the lifted certificate: the base
% bridge on [36,72], the dyadic intervals [60 2^j, 120 2^j] with their
% per-interval gap bounds, and the uniform bound they all exceed.
\newcommand{\coveragefigure}{\begin{tikzpicture}
 \begin{axis}[arxiv axis,width=9.6cm,height=4cm,xmode=log,
  xmin=30,xmax=9000,ymin=.068,ymax=.096,
  xtick={36,60,120,240,480,960,1920,3840},
  xticklabels={$36$,$60$,$120$,$240$,$480$,$960$,$1920$,$3840$},
  ytick={.0729,.08,.09},yticklabels={$0.0729$,$0.08$,$0.09$},scaled y ticks=false,
  xlabel={even length $L$},ylabel={gap bound for $\Delta_L$},
  clip=false]
  \addplot[arxiv bar] coordinates {(36,.090) (72,.090)};
  \node[arxiv note,anchor=south] at (axis cs:51,.0905) {$(36,b_0)$};
  \addplot[arxiv bar] coordinates {(60,.0822) (120,.0822)};
  \addplot[arxiv bar] coordinates {(120,.0749) (240,.0749)};
  \addplot[arxiv bar] coordinates {(240,.0732) (480,.0732)};
  \addplot[arxiv bar] coordinates {(480,.07294) (960,.07294)};
  \addplot[arxiv bar] coordinates {(960,.07293) (1920,.07293)};
  \addplot[arxiv bar] coordinates {(1920,.07293) (3840,.07293)};
  \node[arxiv note,anchor=south west] at (axis cs:62,.0828) {$j=0$};
  \node[arxiv note,anchor=south west] at (axis cs:124,.0755) {$j=1$};
  \node[arxiv note,anchor=south west] at (axis cs:248,.0738) {$j=2$};
  \node[arxiv note,anchor=south west] at (axis cs:2000,.0735) {$j\ge3$; the tail sets the uniform bound};
  \addplot[arxiv cert guide,line width=.7pt] coordinates {(30,.072901771) (9000,.072901771)};
  \node[arxiv cert note,anchor=north west] at (axis cs:31,.0727) {uniform bound};
 \end{axis}
\end{tikzpicture}}



==> figures/diagrams-shared.tex <==
% Diagram and notation definitions shared by the new arXiv manuscript.

\newcommand{\bra}[1]{\langle #1|}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bricknetwork}[1]{%
 \begin{tikzpicture}[x=.43cm,y=.45cm,baseline=-.5ex]
  % the read direction is the flow arrow; no background wash
  \foreach \x in {0,1,2,3}{
   \draw[arxiv boundary] (\x,-.2)--(\x,2.25);}
  \foreach \y in {0,1}{
   \foreach \x in {0,2}{
    \draw[arxiv gate] (\x-.12,\y+.17) rectangle (\x+1.12,\y+.38);}
   \draw[arxiv gate] (.88,\y+.66) rectangle (2.12,\y+.87);
   \draw[arxiv gate] (-.4,\y+.66) rectangle (.12,\y+.87);
   \draw[arxiv gate] (2.88,\y+.66) rectangle (3.4,\y+.87);}
  \draw[arxiv identified] (-.4,-.2) rectangle (3.4,2.25);
  \ifnum#1=1
   \draw[arxiv thermal flow] (3.8,.1)--(3.8,1.9);
  \else
   \draw[arxiv spatial flow] (-.15,2.65)--(3.15,2.65);
  \fi
 \end{tikzpicture}}
\newcommand{\splitgate}{%
 \begin{tikzpicture}[tn,tn centered]
  \draw[phys] (0,-.8)--(0,.8) (1.3,-.8)--(1.3,.8);
  \node[mpo,minimum width=2.2em,minimum height=.5em] at (.65,0) {};
 \end{tikzpicture}}
\newcommand{\bondends}{%
 \begin{tikzpicture}[tn,tn centered]
  \draw[phys] (0,-.8)--(0,.8) (2,-.8)--(2,.8);
  \draw[mpored] (0,0)--(2,0);
  \node[mpo] at (0,0) {$A_\gamma$};
  \node[mpo] at (2,0) {$A_\gamma$};
 \end{tikzpicture}}
\newcommand{\torusgluing}{%
 \begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize]
  \def\c{.28}\def\g{.12}
  \foreach \a in {0,1}{\foreach \b in {0,1}{
   \tnpatch{{\a*(2*\c+\g)}}{{1.9+\b*(\c+\g)}}{2}{1}{\c}}}
  \foreach \b in {0,1}{
   \tnpatch{5.1}{{1.9+\b*(\c+\g)}}{4}{1}{\c}}
  \foreach \a in {0,1}{
   \tnpatch{{\a*(2*\c+\g)}}{.1}{2}{2}{\c}}
  \tnpatch{5.1}{.1}{4}{2}{\c}
  \node[anchor=north] at (.62,1.85) {$Z_n(\beta)^4$};
  \node[anchor=north] at (5.66,1.85) {$Z_{2n}(\beta)^2$};
  \node[anchor=north] at (.62,.05) {$Z_n(2\beta)^2$};
  \node[anchor=north] at (5.66,.05) {$Z_{2n}(2\beta)$};
  \draw[arxiv spatial flow] (1.45,2.2)--(4.9,2.2)
   node[midway,above,text=black] {$\times\Ps(n,\beta)^2$};
  \draw[arxiv spatial flow] (1.45,.38)--(4.9,.38)
   node[midway,above,text=black] {$\times\Ps(n,2\beta)$};
  \draw[arxiv thermal flow] (.62,1.48)--(.62,.8)
   node[midway,right,text=black] {$\times\Pt(n,\beta)^2$};
  \draw[arxiv thermal flow] (5.66,1.48)--(5.66,.8)
   node[midway,left,text=black] {$\times\Pt(2n,\beta)$};
 \end{tikzpicture}}


% Periodic MPS norm (#1=0) and one-bond energy (#1=1): the ket row and its
% conjugate row each close into a virtual loop drawn clear of the tensors.
\newcommand{\seedmps}[1]{\tikz[tn,tn centered]{
 \foreach \y/\s in {.9/1,-.9/-1}{
  \draw[ring] (-1.1,\y)--(-1.1,{\y+\s*.55})
   --(6.7,{\y+\s*.55})--(6.7,\y)--cycle;}
 \foreach \x in {0,2.2,5.6}{
  \draw[phys] (\x,-.9)--(\x,.9);}
 \tndots{3.9}{.9}\tndots{3.9}{-.9}
 \ifnum#1=1
  \node[sym,fill=mpoblue!14,minimum width=3.4em,minimum height=.65em,inner sep=0pt]
   at (1.1,0) {$h$};
 \fi
 \foreach \x in {0,2.2,5.6}{
  \node[mpo,fill=white] at (\x,.9) {$A$};
  \node[mpo,fill=white] at (\x,-.9) {$A$};}}}


% A reflection-positive bond term with explicit factors: #1 on the left site,
% its mirror image #2 on the right site, across the mirror cut (F = I when
% the two labels agree).
\newcommand{\rpbondpic}[2]{\tikz[tn,tn centered]{
 \draw[phys] (0,-.85)--(0,.85);
 \draw[phys] (3.4,-.85)--(3.4,.85);
 \draw[arxiv bond] (0,0)--(3.4,0);
 \draw[arxiv mirror] (1.7,-1)--(1.7,1);
 \node[xop] at (0,0) {$#1$};
 \node[xop] at (3.4,0) {$#2$};}}
% The bond mirror of the cell theorem: C_alpha against its reflection F C_alpha F.
\newcommand{\scopebond}{\rpbondpic{C_\alpha}{FC_\alpha F}}


\newcommand{\smI}{I}
\newcommand{\smF}{\mathcal F}
\newcommand{\smZ}[1]{Z_{#1}^{(M)}}
\newcommand{\smT}{T_{\beta,M}}
\newcommand{\smD}{\mathcal D_M}
\newcommand{\smnorm}[1]{\left\lVert #1\right\rVert}


\newcommand{\obccap}[2]{%
 \tnchain[capl={\bar v_\beta},capr={#2}]{#1}}
\newcommand{\obcW}{%
 \tnchain[node=mpo,legs,capl={\bar v_\beta},capr={v_\beta}]
 {W_\beta,\cdots,W_\beta}}



% Six-site ring glyph, with a spatial twist on one closing bond when #1=1.
\newcommand{\seedring}[1]{\tikz[baseline=-.6ex,x=1em,y=1em]{
 \draw[black!70,line width=.45pt] (90:1)--(30:1)--(-30:1)
  --(-90:1)--(-150:1)--(150:1)--cycle;
 \ifnum#1=1
  \draw[mpored,line width=1.6pt] (150:1)--(90:1);
  \node[overlay,font=\scriptsize,text=mpored] at (-.8,1.15) {$\pi$};
 \fi
 \foreach \a in {90,30,-30,-90,-150,150}{
  \filldraw[draw=black!70,fill=white,line width=.45pt] (\a:1) circle (.12);}}}

% Extremal twelfth-moment weights and their sixth powers, not an observed spectrum.
\newcommand{\seedweightbars}{\begin{tikzpicture}[x=1cm,y=.55cm,baseline=-.5ex]
 % half-height bars with the labels beside them, so the glyph costs three text lines
 \fill[arxiv leading weight] (0,0) rectangle (.4,.9881);
 \fill[arxiv remainder weight] (.8,0) rectangle (1.2,.0777);
 \draw[arxiv guide] (-.1,.9881)--(1.3,.9881);
 \node[arxiv label,anchor=west,inner sep=2pt] at (1.3,.9881) {$\ell^{12}$};
 \node[arxiv label,anchor=west,inner sep=2pt] at (1.3,.12) {$m_J-\ell^{12}$};
 \draw[arxiv gray flow] (3.1,.5)--(4.1,.5)
  node[midway,above,arxiv label,inner sep=1.5pt] {$u\mapsto u^6$};
 \fill[arxiv leading weight] (4.6,0) rectangle (5,.9305);
 \fill[arxiv remainder weight] (5.4,0) rectangle (5.8,.000001);
 \node[arxiv label,anchor=west,inner sep=2pt] at (5.9,.9305) {$\ell^{72}$};
 \draw[arxiv baseline] (-.1,0)--(1.3,0) (4.5,0)--(5.9,0);
\end{tikzpicture}}

% The four established coupling/squaring steps, in the talk's two-lane layout.
% Rows are packed to 1.05 cm, and the thermal lane sits half a row above
% the spatial one, so the staircase fits a column without a tall gap.
\newcommand{\pbcsteps}{\begin{prooflanes}\def\lanedy{1.05}
 \lanebound{s}{ps0}{0}{0}{$\Ps(n,\beta)\ge1-p$}
 \lanebound{t}{pt0}{1}{0}{$\Pt(2n,\beta)\ge1-q$}
 \lanebound{so}{ps1}{0}{1}{$\Ps(n,2\beta)\ge(1-p)^2(1-q)$}
 \lanebound{s}{ps2}{0}{2}{$\Ps(2n,2\beta)\ge1-p'$}
 \lanebound{to}{pt1}{1}{2.5}{$\Pt(4n,\beta)\ge(1-q)^2(1-p')$}
 \lanebound{t}{pt2}{1}{3.5}{$\Pt(4n,2\beta)\ge1-q'$}
 \lanemove{ps0}{ps1}{1}{identity}\laneuse{pt0}{1}
 \lanemove[mpored]{ps1}{ps2}{2}{square in space}
 \lanemove{pt0}{pt1}{3}{identity}\laneuse{ps2}{3}
 \lanemove[mpoblue]{pt1}{pt2}{4}{square in time}
\end{prooflanes}}

% Adapted from the proof-strategy slide; errors are schematic, not the seed orbit.
\newcommand{\strategystairs}{\begin{tikzpicture}[x=.8cm,y=.8cm,
 every node/.style={arxiv label,inner sep=1pt}]
 \draw[arxiv dotted guide] (0,0)--(3.3,2.1);
 \foreach \x/\y in {0/0,1.65/1.05}{
  \draw[arxiv thermal flow,line width=1pt] (\x,\y+.04)--(\x,\y+1.01);
  \draw[arxiv spatial flow,line width=1pt,densely dashed]
   (\x+.04,\y+1.05)--(\x+1.61,\y+1.05);}
 \foreach \x/\y in {0/0,0/1.05,1.65/1.05,1.65/2.1,3.3/2.1}{
  \node[arxiv point] at (\x,\y) {};}
 \foreach \x/\lab in {0/n_0,1.65/2n_0,3.3/4n_0}{
  \node[anchor=north] at (\x,-.16) {$\lab$};}
 \foreach \y/\lab in {0/\beta_0,1.05/2\beta_0,2.1/4\beta_0}{
  \node[anchor=east] at (-.15,\y) {$\lab$};}
 \node[anchor=west,fill=white] at (.12,.22) {$\varepsilon$};
 \node[anchor=west,fill=white] at (1.8,1.28) {$\approx\varepsilon^2$};
 \node[anchor=south] at (3.3,2.22) {$\approx\varepsilon^4$};
 % key: each move with the arrow that draws it, close to the staircase
 \draw[arxiv thermal flow,line width=1pt] (4.15,1.9)--(4.15,2.35);
 \node[text=mpoblue,anchor=west] at (4.3,2.12) {double $\beta$};
 \node[anchor=west] at (4.3,1.68) {$\rho_n(\beta)^2\propto\rho_n(2\beta)$};
 \draw[arxiv spatial flow,line width=1pt,densely dashed] (3.95,.95)--(4.4,.95);
 \node[text=mpored,anchor=west] at (4.5,.95) {double $n$};
 \node[anchor=west] at (4.3,.5) {$\sigma_n^2\propto\sigma_{2n}$};
\end{tikzpicture}}

% ------------------------------------------------- Supplemental Material glyphs
% One site of the brickwork network through three slices, read along space:
% the odd-bond labels q_t enter from the left and the even-bond labels p_t
% leave to the right; the loop is the physical trace that gives F_{pq}.
\newcommand{\sitetrace}{\tikz[tn,tn centered,font=\scriptsize]{
 \draw[phys,ring] (0,-1.75)--(0,1.75)--(2.9,1.75)--(2.9,-1.75)--cycle;
 \foreach \y/\p/\q in {-1.05/p_0/q_0,0/p_1/q_1,1.05/p_2/q_2}{
  \draw[arxiv bond] (-1.05,{\y-.22})--(0,{\y-.22});
  \draw[arxiv bond] (0,{\y+.22})--(1.05,{\y+.22});
  \node[xvertex] at (0,{\y-.22}) {};
  \node[xvertex] at (0,{\y+.22}) {};
  \node[anchor=east,inner sep=1pt] at (-1.05,{\y-.22}) {$\q$};
  \node[anchor=west,inner sep=1pt] at (1.05,{\y+.22}) {$\p$};}}}

% One site of the brickwork network traced through M=2 slices, read along
% space: on each slice the odd-bond factor A_{a_t} enters from the left and the
% even-bond factor A_{b_t} leaves to the right; the closed physical loop is the
% trace, so the picture is the matrix element F_{ba} of the main text.
\newcommand{\sitetraceab}{\tikz[tn,tn centered,font=\scriptsize]{
 \draw[phys,ring] (0,-1.2)--(0,1.2)--(2.7,1.2)--(2.7,-1.2)--cycle;
 \foreach \y/\b/\a in {-.55/b_1/a_1,.55/b_2/a_2}{
  \draw[arxiv bond] (-1.05,{\y-.22})--(0,{\y-.22});
  \draw[arxiv bond] (0,{\y+.22})--(1.05,{\y+.22});
  \node[xvertex] at (0,{\y-.22}) {};
  \node[xvertex] at (0,{\y+.22}) {};
  \node[anchor=east,inner sep=1pt] at (-1.05,{\y-.22}) {$\a$};
  \node[anchor=west,inner sep=1pt] at (1.05,{\y+.22}) {$\b$};}}}

% \capbars[yunit]{h1,h2,...}{cap}: twelfth-power weights filled up to a cap
% (dashed) with the remaining mass in one smaller entry; the extremal
% configuration of the capped-mass bound.
\newcommand{\capbars}[3][1.1em]{\tikz[baseline=0pt,x=.5em,y=#1]{
 \foreach \h [count=\i from 0] in {#2}{
  \fill[arxiv leading weight] ({1.15*\i},0) rectangle ++(.8,\h);
  \xdef\capn{\i}}
 \draw[arxiv guide] (-.2,#3)--({1.15*\capn+1},#3);
 \draw[arxiv baseline] (-.25,0)--({1.15*\capn+1.05},0);}}

% Twelfth-power weights of K at the base seed: one dominant J eigenvalue,
% the J remainder, and the three identical N lists.
\newcommand{\sectorspectrum}{\tikz[baseline=0pt,x=.34em,y=1.1em]{
 \fill[arxiv leading weight] (0,0) rectangle ++(.78,1);
 \foreach \h [count=\i] in {.35,.2}{\fill[arxiv remainder weight] (\i,0) rectangle ++(.78,\h);}
 \foreach \h [count=\i from 3] in {.58,.58,.58,.3,.3,.3}{\fill[arxiv bulk weight] (\i,0) rectangle ++(.78,\h);}
 \draw[arxiv baseline] (-.2,0)--(9,0);
}}

% The filter F_N against its certified total B_N: the level is crossed at
% +-V and no eigenvalue of the N lists can sit on the shaded exterior rays.
\newcommand{\filterglyph}{\tikz[baseline=0pt,x=1.7em,y=1.1em,line width=.45pt]{
 \clip (-1.05,-.08) rectangle (1.05,1.05);
 \fill[arxiv exclude band] (-1.05,0) rectangle (-.872,1.05);
 \fill[arxiv exclude band] (.872,0) rectangle (1.05,1.05);
 \draw[arxiv baseline] (-1.05,0)--(1.05,0);
 \draw[arxiv guide] (-1.05,.535)--(1.05,.535);
 \draw[arxiv curve,domain=-1:1,samples=161,smooth]
  plot (\x,{(\x^4)*((12-394*\x*\x+1000*\x^4)/300)^2});}}

% The six exact rational steps on a logarithmic scale: data of Table sm:tab:orbit.
\newcommand{\defectladder}{\begin{tikzpicture}[x=1.05cm,y=1.6cm,font=\footnotesize]
 \def\ps{-1.320,-1.218,-1.163,-1.146,-1.198,-1.425,-2.072}
 \def\qs{-.741,-.761,-.787,-.839,-.976,-1.350,-2.258}
 \draw[arxiv guide] (0,-2)--(6,-2)
  node[right,arxiv note] {$10^{-2}$};
 \draw[arxiv dotted guide] (0,-.895)--(6,-.895)
  node[right,arxiv note] {$\varepsilon_*$};
 \foreach \v [count=\i from 0] in \ps{\ifnum\i>0 \draw[arxiv series,mpored] ({\i-1},\pl)--(\i,\v);\fi
  \fill[mpored] (\i,\v) circle[radius=1.3pt]; \xdef\pl{\v}}
 \foreach \v [count=\i from 0] in \qs{\ifnum\i>0 \draw[arxiv series,mpoblue] ({\i-1},\ql)--(\i,\v);\fi
  \fill[mpoblue] (\i,\v) circle[radius=1.3pt]; \xdef\ql{\v}}
 \node[mpored,anchor=north] at (2.5,-1.19) {$p_j$ (spatial)};
 \node[mpoblue,anchor=south] at (1.5,-.76) {$q_j$ (thermal)};
 \foreach \n [count=\i from 0] in {36,72,144,288,576,1152,2304}{
  \node[arxiv note] at (\i,-2.42) {$\n$};}
 \node[arxiv note,anchor=east] at (-.25,-2.42) {$n_j$};
\end{tikzpicture}}

% Interpolation between dyadic scales, adapted from the talk: the unknown
% length L is bounded from above at beta_j by the torus on its left and from
% below at 2 beta_j by the torus on its right.
\newcommand{\dyadicinterval}{\begin{tikzpicture}[x=1cm,y=.75cm,
 every node/.style={arxiv label,inner sep=1pt}]
 \draw[black!25,line width=.45pt] (-.3,0)--(4.4,0) (-.3,1.8)--(4.4,1.8);
 \foreach \x/\l in {0/n_j,3.6/2n_j}{
  \draw[black!25,line width=.45pt] (\x,-.2)--(\x,2.2);
  \node[anchor=north] at (\x,-.25) {$\l$};}
 \node[anchor=east] at (-.35,0) {$\beta_j$};
 \node[anchor=east] at (-.35,1.8) {$2\beta_j$};
 \draw[arxiv dotted guide] (0,0)--(3.6,1.8);
 \draw[tncert,line width=1pt] (1.9,-.2)--(1.9,2.2);
 \node[anchor=north,arxiv cert note] at (1.9,-.25) {$L$};
 \draw[arxiv spatial flow,line width=.7pt] (.12,0)--(1.78,0);
 \draw[arxiv spatial flow,line width=.7pt] (3.48,1.8)--(2.02,1.8);
 \node[arxiv point] at (0,0) {};
 \node[arxiv point] at (3.6,1.8) {};
 \node[arxiv point,fill=tncert] at (1.9,0) {};
 \node[arxiv point,fill=tncert] at (1.9,1.8) {};
 \node[anchor=south,text=mpored,inner sep=1pt,fill=white] at (.95,.07) {power $L/n_j$};
 \node[anchor=south west,text=mpored,inner sep=1pt,fill=white] at (2.05,1.86) {power $2n_j/L$};
 \node[anchor=west,arxiv note] at (2.45,.62) {doubling};
\end{tikzpicture}}

% Word-sized dyadic interval: the two known tori (gray points, at (n_j, beta_j)
% below and (2n_j, 2beta_j) above) bound the thermal purity at the target length
% L (teal) from either side by the power-sum inequality along the length axis
% (red). Unlabeled so that it stays one line tall; the prose names the points.
\newcommand{\interpolationglyph}{\tikz[baseline=-.1em,x=1em,y=.8em]{
 \draw[arxiv baseline] (-.15,0)--(2.75,0) (-.15,.75)--(2.75,.75);
 \draw[arxiv series,tncert] (1.3,-.1)--(1.3,.87);
 \draw[arxiv small arrow,mpored] (.2,0)--(1.18,0);
 \draw[arxiv small arrow,mpored] (2.4,.75)--(1.42,.75);
 \node[arxiv point,inner sep=.9pt] at (0,0) {};
 \node[arxiv point,inner sep=.9pt] at (2.6,.75) {};
 \node[arxiv point,inner sep=.9pt,fill=tncert] at (1.3,0) {};
 \node[arxiv point,inner sep=.9pt,fill=tncert] at (1.3,.75) {};
}}



==> figures/diagrams-trotter.tex <==
% Diagrams for the finite-Trotter and doubling section of the Supplemental Material.

% Two-site column of the brickwork network through three slices (dashed top and
% bottom edges identified): the two sites share the even-bond labels b_{k,t} on the
% rungs and carry the odd-bond labels c_{k-1,t}, c_{k,t} on their outer legs; the mirror
% maps the left site onto the right one, so the column is F^T F summed over b.
\newcommand{\twositecolumn}{\begin{tikzpicture}[x=1em,y=1em,line width=.45pt,
 font=\scriptsize,baseline={([yshift=-.5ex]current bounding box.center)}]
 \fill[mpored!8] (-.9,-1.75) rectangle (4.9,1.75);
 \draw[arxiv identified] (-.9,-1.75)--(4.9,-1.75) (-.9,1.75)--(4.9,1.75);
 \draw[phys] (0,-1.75)--(0,1.75);
 \draw[phys] (4,-1.75)--(4,1.75);
 \draw[arxiv mirror] (2,-2.15)--(2,2.15);
 \foreach \y/\t in {-1.05/0,0/1,1.05/2}{
  \draw[arxiv bond] (0,{\y+.22})--(4,{\y+.22});
  \draw[arxiv bond] (-1.5,{\y-.22})--(0,{\y-.22});
  \draw[arxiv bond] (4,{\y-.22})--(5.5,{\y-.22});
  \node[xvertex] at (0,{\y+.22}) {}; \node[xvertex] at (4,{\y+.22}) {};
  \node[xvertex] at (0,{\y-.22}) {}; \node[xvertex] at (4,{\y-.22}) {};
  \node[text=mpored,anchor=south,inner sep=1pt,fill=white] at (2,{\y+.27}) {$b_{k,\t}$};
  \node[anchor=east,inner sep=1pt] at (-1.5,{\y-.22}) {$c_{k-1,\t}$};
  \node[anchor=west,inner sep=1pt] at (5.5,{\y-.22}) {$c_{k,\t}$};}
 \node[anchor=north,inner sep=2pt] at (0,-1.8) {$\smF_{b_kc_{k-1}}$};
 \node[anchor=north,inner sep=2pt] at (4,-1.8) {$\smF_{b_kc_k}$};
\end{tikzpicture}}

% The ring of alternating F^T and F columns whose trace is Z^{(M)}_{2N}.
\newcommand{\columnring}{\tnchain[ring]{\smF^{\mathsf T},\smF,\cdots,\smF^{\mathsf T},\smF}}

% The square of side S_1 = a_1 + a_2 + a_3 cut by the weights (grays, as all
% weights): the dark diagonal blocks have area S_2, the light off-diagonal blocks
% have area S_1^2 - S_2.
\newcommand{\pairsquare}{\tikz[baseline={(0,.4)},x=2.2em,y=2.2em,line width=.35pt]{
 \foreach \l/\h in {0/.5,.5/.8,.8/1}{
  \foreach \L/\H in {0/.5,.5/.8,.8/1}{
   \ifdim\l pt=\L pt \fill[arxiv leading weight] (\l,\L) rectangle (\h,\H);
   \else \fill[arxiv remainder weight] (\l,\L) rectangle (\h,\H);\fi}}
 \draw[white,line width=.45pt] (.5,0)--(.5,1) (.8,0)--(.8,1) (0,.5)--(1,.5) (0,.8)--(1,.8);
 \draw[arxiv axis line] (0,0) rectangle (1,1);}}

% A brickwork patch of fixed width (four sites) and height beta, sliced into #3
% rows: \refinedpatch{x}{y}{rows}.
\newcommand{\refinedpatch}[3]{\begin{scope}[shift={(#1,#2)}]
 \draw[arxiv identified] (0,0) rectangle (1.28,.64);
 \foreach \i in {1,...,4}{\draw[line width=.45pt] ({(\i-.5)*.32},0)--({(\i-.5)*.32},.64);}
 \foreach \j in {1,...,#3}{
  \draw[line width=.45pt] (0,{(\j-.5)*.64/#3})--(1.28,{(\j-.5)*.64/#3});
  \foreach \i in {1,...,4}{\filldraw[fill=mpoblue,line width=.35pt]
   ({(\i-.5)*.32-.045},{(\j-.5)*.64/#3-.045}) rectangle ++(.09,.09);}}
\end{scope}}

% At one fixed (L, beta), the brickwork network is refined, M = 1, 2, 4, ..., and
% converges to the exact Gibbs operator; the doubling argument acts only on the
% limits.
\newcommand{\limitfirst}{\begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize]
 \foreach \i/\rows/\lab in {0/1/{M=1},1/2/{M=2},2/4/{M=4}}{
  \refinedpatch{\i*1.75}{0}{\rows}
  \node[anchor=north,arxiv note] at ({\i*1.75+.64},-.08) {$\lab$};}
 \foreach \x in {1.33,3.08}{\draw[arxiv gray flow] (\x,.32)--(\x+.37,.32);}
 \draw[arxiv gray flow] (4.83,.32)--(6.05,.32) node[midway,above,arxiv note] {$M\to\infty$};
 \node[gibbs,minimum width=1.28cm,minimum height=.64cm] at (6.74,.32) {};
 \node at (6.74,.32) {$e^{-\beta H_L}$};
 \node[anchor=north,arxiv note] at (6.74,-.08) {exact};
\end{tikzpicture}}

% One asymmetric doubling step with the identity or inequality used on each move.
\newcommand{\asymsteps}{\begin{prooflanes}[5.4]\def\lanedy{1.05}
 \lanebound{s}{as0}{0}{0}{$\Ps(n,\beta)\ge1-p$}
 \lanebound{t}{at0}{1}{0}{$\Pt(2n,\beta)\ge1-q$}
 \lanebound{so}{as1}{0}{1}{$\Ps(n,2\beta)\ge(1-p)^2(1-q)=1-z(p,q)$}
 \lanebound{s}{as2}{0}{2}{$\Ps(2n,2\beta)\ge1-f(z(p,q))=1-p'$}
 \lanebound{to}{at1}{1}{2.5}{$\Pt(4n,\beta)\ge(1-q)^2(1-p')=1-z(q,p')$}
 \lanebound{t}{at2}{1}{3.5}{$\Pt(4n,2\beta)\ge1-f(z(q,p'))=1-q'$}
 \lanemove{as0}{as1}{1}{\eqref{sm:eq:coupling}, drop $\Pt(n,\beta)^2\le1$}\laneuse{at0}{1}
 \lanemove[mpored]{as1}{as2}{2}{\eqref{sm:eq:two-squares}, $f$ monotone}
 \lanemove{at0}{at1}{3}{\eqref{sm:eq:coupling}, drop $\Ps(2n,\beta)^2\le1$}\laneuse{as2}{3}
 \lanemove[mpoblue]{at1}{at2}{4}{\eqref{sm:eq:two-squares}, $f$ monotone}
 \lanetag[above]{as0}{given}
 \lanetag[above]{at0}{given}
\end{prooflanes}}

% The gate I - tau h split into matching bond factors C_gamma on its two sites,
% joined by the summed bond label (space, red): the real bond-reflection-positive form.
\newcommand{\bondendsA}{\begin{tikzpicture}[tn,tn centered]
 \draw[phys] (0,-.8)--(0,.8) (2,-.8)--(2,.8);
 \draw[mpored] (0,0)--(2,0);
 \node[xop] at (0,0) {$A_\gamma$};
 \node[xop] at (2,0) {$A_\gamma$};
\end{tikzpicture}}

% One cell through two slices of the reflection-positive cell model, bottom to
% top on each slice: the reflection F (gray tick), the odd-bond factor (red), F
% again, the on-site factor O (blue, imaginary time), and the even-bond factor;
% the trace gives F_{pq}.
\newcommand{\cellsitetrace}{\tikz[tn,tn centered,font=\scriptsize]{
 \draw[phys,ring] (0,-1.75)--(0,1.75)--(2.9,1.75)--(2.9,-1.75)--cycle;
 \foreach \y/\p/\q in {-.85/p_0/q_0,.85/p_1/q_1}{
  \draw[arxiv bond] (-1.05,{\y-.3})--(0,{\y-.3});
  \draw[arxiv bond] (0,{\y+.5})--(1.05,{\y+.5});
  \draw[arxiv boundary] (-.32,{\y-.55})--(.32,{\y-.55});
  \node[xvertex] at (0,{\y-.3}) {};
  \draw[arxiv boundary] (-.32,{\y-.05})--(.32,{\y-.05});
  \node[mpo,minimum size=.44em,inner sep=0pt] at (0,{\y+.2}) {};
  \node[xvertex] at (0,{\y+.5}) {};
  \node[anchor=east,inner sep=1pt] at (-1.05,{\y-.3}) {$\q$};
  \node[anchor=west,inner sep=1pt] at (1.05,{\y+.5}) {$\p$};}}}

% The odd cell of the reflection-positive cell model through two slices: the
% same worldline as \cellsitetrace with the two F ticks around the even-bond
% factor instead of the odd one (F A_p F O A_q, using FO = OF). The closed loop
% is a trace, so moving F around it (F^2 = I) leaves F_{pq} unchanged and both
% sublattices share one transfer matrix. Display glyph beside \cellsitetrace.
\newcommand{\oddcellsitetrace}{\tikz[tn,tn centered,font=\scriptsize]{
 \draw[phys,ring] (0,-1.75)--(0,1.75)--(2.9,1.75)--(2.9,-1.75)--cycle;
 \foreach \y/\p/\q in {-.85/p_0/q_0,.85/p_1/q_1}{
  \draw[arxiv bond] (-1.05,{\y-.6})--(0,{\y-.6});
  \draw[arxiv bond] (0,{\y+.3})--(1.05,{\y+.3});
  \node[xvertex] at (0,{\y-.6}) {};
  \node[mpo,minimum size=.44em,inner sep=0pt] at (0,{\y-.28}) {};
  % the ticks protrude past the vertex and the box so that their new place shows
  \draw[arxiv boundary] (-.32,{\y+.02})--(.32,{\y+.02});
  \node[xvertex] at (0,{\y+.3}) {};
  \draw[arxiv boundary] (-.32,{\y+.58})--(.32,{\y+.58});
  \node[anchor=east,inner sep=1pt] at (-1.05,{\y-.6}) {$\q$};
  \node[anchor=west,inner sep=1pt] at (1.05,{\y+.3}) {$\p$};}}}

% One term of X^k - Y^k = sum_r X^{k-1-r} (X - Y) Y^r: k - 1 links of norm at most
% K and one link X - Y, so the term has norm at most K^{k-1} ||X - Y||.
\newcommand{\telescopechain}{\tikz[tn,tn centered]{
 \tnchainpath[node=sym,name=t,item={minimum height=1.1em}]{X,\cdots,X,X-Y,Y,\cdots,Y}
 \node[sym,fill=black!25,minimum height=1.1em] at (t-4) {$X-Y$};
 \draw[arxiv baseline]
  ([yshift=-.3em]t-1.south west)--([yshift=-.3em]t-3.south east)
  node[midway,below,inner sep=1.5pt,arxiv note] {$k-1-r$};
 \draw[arxiv baseline]
  ([yshift=-.3em]t-5.south west)--([yshift=-.3em]t-7.south east)
  node[midway,below,inner sep=1.5pt,arxiv note] {$r$};}}

% The squaring map f(z) = z^2/[2(1-z)^2] on 0 <= z <= .3 lies under the diagonal
% (gray: f acts on spatial and thermal weights alike).
\newcommand{\fbelowdiag}{\tikz[baseline=0pt,x=3.3em,y=3.3em,line width=.45pt]{
 \draw[arxiv baseline] (0,0)--(.3,0) (0,0)--(0,.3);
 \draw[arxiv dotted guide] (0,0)--(.3,.3);
 \draw[arxiv curve,domain=0:.3,samples=25,smooth] plot (\x,{\x*\x/(2*(1-\x)*(1-\x))});}}

% The integer check behind one table entry: the exact value D f (gray) lies on the
% grid interval (a - 1, a], so the stored entry a (teal) is its ceiling.
\newcommand{\ceilcheck}{\tikz[baseline=-.6ex,x=3.6em,y=.8em,line width=.45pt,font=\scriptsize]{
 \draw[arxiv axis line] (-.4,0)--(1.4,0);
 \draw[arxiv axis line] (0,-.14)--(0,.14) (1,-.14)--(1,.14);
 \node[anchor=north,inner sep=1.5pt,arxiv note] at (0,-.14) {$a_{j+1}-1$};
 \node[anchor=north,inner sep=1.5pt,arxiv cert note] at (1,-.14) {$a_{j+1}$};
 \draw[black!55] (0,0) circle[radius=.14em];
 \fill[arxiv leading weight] (.58,0) circle[radius=.14em];
 \node[anchor=south,inner sep=1.5pt,arxiv note] at (.58,.1) {$Df$};
 \draw[arxiv small arrow] (.66,.2)--(.94,.2);
 \fill[tncert] (1,0) circle[radius=.14em];}}

% Energy levels with the gap (teal, the certified quantity) and their Gibbs weights
% (gray): the purity is at most the largest weight w_0, and w_0 above one half
% (dashed) leaves no room for a second weight of the same size.
\newcommand{\levelweights}{\tikz[baseline={([yshift=-.5ex]current bounding box.center)},
 x=1.8em,y=2.8em,line width=.45pt,font=\scriptsize]{
 \draw (0,0)--(1,0);
 \foreach \y in {.55,.75,.9}{\draw[arxiv axis line] (0,\y)--(1,\y);}
 \node[anchor=east,inner sep=2pt,arxiv note] at (0,0) {$E_0$};
 \node[anchor=east,inner sep=2pt,arxiv note] at (0,.55) {$E_1$};
 \draw[tncert,line width=1pt] (1.15,0)--(1.15,.55);
 \node[anchor=west,inner sep=2pt,arxiv cert note] at (1.15,.27) {$\Delta_L$};
 \draw[arxiv gray flow] (2.3,.45)--(3.2,.45);
 \node[anchor=south,inner sep=2pt,arxiv note] at (2.75,.47) {$e^{-\beta_jE}$};
 \draw[arxiv baseline] (3.4,0)--(4.95,0);
 \fill[arxiv leading weight] (3.5,0) rectangle (3.85,.97);
 \fill[arxiv remainder weight] (4,0) rectangle (4.35,.03);
 \fill[arxiv remainder weight] (4.5,0) rectangle (4.85,.015);
 \draw[arxiv guide] (3.4,.5)--(4.95,.5)
  node[anchor=west,inner sep=2pt,arxiv note] {$\tfrac12$};
 \node[anchor=south,inner sep=2pt,arxiv note] at (3.675,.97) {$w_0$};
 \node[anchor=south,inner sep=2pt,arxiv note] at (4.175,.05) {$w_1$};}}

% \trendline[floor]{min}{max}{v0,v1,...}: word-sized line of the values with gray
% end marks; an optional floor draws the uniform bound (teal, dashed) they approach.
\newcommand{\trendline}[4][]{\tikz[baseline=0pt,x=.75em,y=.9em,line width=.45pt]{
 \foreach \tv [count=\ti from 0] in {#4}{
  \pgfmathsetmacro\ty{(\tv-(#2))/((#3)-(#2))}
  \ifnum\ti=0 \fill[black!70] (0,\ty) circle[radius=.09em];
  \else\draw[black!70] ({\ti-1},\tpy)--(\ti,\ty);\fi
  \xdef\tpy{\ty}\xdef\tlx{\ti}}
 \fill[black!70] (\tlx,\tpy) circle[radius=.09em];
 \if\relax\detokenize{#1}\relax\else
  \pgfmathsetmacro\tfl{((#1)-(#2))/((#3)-(#2))}
  \draw[arxiv cert guide] (-.2,\tfl)--(\tlx+.3,\tfl);\fi}}

